Harnessing Large Language Models as Post-hoc Correctors

As Machine Learning (ML) models grow in size and demand higher-quality training data, the expenses associated with re-training and fine-tuning these models are escalating rapidly. Inspired by recent impressive achievements of Large Language Models (LLMs) in different fields, this paper delves into the question: can LLMs efficiently improve an ML's performance at a minimal cost? We show that, through our proposed training-free framework LlmCorr, an LLM can work as a post-hoc corrector to propose corrections for the predictions of an arbitrary ML model. In particular, we form a contextual knowledge database by incorporating the dataset's label information and the ML model's predictions on the validation dataset. Leveraging the in-context learning capability of LLMs, we ask the LLM to summarise the instances in which the ML model makes mistakes and the correlation between primary predictions and true labels. Following this, the LLM can transfer its acquired knowledge to suggest corrections for the ML model's predictions. Our experimental results on text analysis and the challenging molecular predictions show that \model improves the performance of a number of models by up to 39%.

==> pages/are_llms_classifiers.tex <==
\input{tables/table-preliminary-performance}

After a comprehensive demonstration of \model's significance working as a post-hoc corrector, one question raised to us: Is the reason behind \model's outstanding performance is because the LLM understands how to correct the ML model's predictions or the LLM has the inherent capability to predict molecule's properties? 
To answer this question, we perform another set of empirical studies. 
In particular, we design predictor prompts to ask LLMs to directly predict the molecule's properties without any information about the ML model's predictions. 

\subsection{Predictor Prompt Engineering}
\label{subsec:predictor_prompt:engineering}

\textbf{Zero-shot Prompting}.
The first set of prompts (\IP, \IE) simply provides the LLM with molecule and task descriptions and asks it to generate the desired output with a desired format without any prior training or knowledge on the task, as illustrated in Figure~\ref{fig:zero_shot_prompt}. 
The only guidance we provide to the LLM is instruction, which tells about a little background context. 
Particularly, \IP only asks the LLM to provide predictions, while \IE further asks for explanations, which may ask the LLM to clarify the thought process in explanation generation and provide helpful evidence to help users to understand the given prediction. 
In addition, if we fill out the description of \IP and \IE, which derives \IPD and \IPD prompts. 

\smallskip
\noindent
\textbf{Few-shot Prompting}.
The second kind of prompt (\FS) that we propose provides the LLM with a small number of examples of the task, along with the desired outputs~\cite{BMRS20}.
The model then learns from these examples to perform the task on new inputs. 
This approach can be categorised as a simple in-context learning (ICL) technique, 
An example prompt template is shown in Figure~\ref{fig:fs_prompt}. 
In this work, we do not discuss the \FS prompts 

We note there are also some popular recent ICL techniques, \eg, Chain-of-thought (CoT)~\cite{WWSBIXCLZ22}, Tree-of-thought (ToT)~\cite{YYZSGCN23}, Graph-of-thought (GoT)~\cite{BBKG23} and Retrieval Augmented Generation (RaG)~\cite{LPPP20}, which are theoretically available to support complicated tasks and include large knowledge context. 
However, our initial experiments showed that methods, \eg, CoT, ToT and GoT, perform much worse for molecule property prediction tasks due to the significant difficulties in designing proper chain thoughts without solid expertise.
RaG implementations that we tested are unstable and slow with query, and they fall short of the relatively simpler \FS's performance. 
We argue it is caused by the unqualified information retrieval system, and we will discuss it in the future work discussion section. 

\subsection{Results - LLMs work as Predictors}

\textbf{Observation 5: }
\textbf{LLMs are not competitive predictors.}
From the results of Table~\ref{table:performance_llms_as_predictors}, we can observe that the LLM can generate predictions about the molecule's property.
However, LLM's performances are not significantly competitive compared with the ML models' performance, as shown in Table~\ref{table:performance_llms_as_correctors}. 
Hence, we argue existing LLMs are not competitive predictors and employing LLMs as effective predictors is still an open challenge. 

\smallskip\noindent
\textbf{Observation 6: }
\textbf{Description is not an effective approach to encode graphs for LLMs.}
By comparing the performance of $\model_{\IP}$ vs. $\model_{\IPD}$ and $\model_{\IE}$ vs. $\model_{\IED}$ of Table~\ref{table:performance_llms_as_predictors}, we can find that adding description into the prompt harm the performance. 
In addition, we statistic the consistency of responses (whether the LLM answers our questions strictly following the required format) generated by the LLM in Figure~\ref{fig:consistency}. 
We can find that adding a description will heavily decrease the response's consistency.
We argue it is due the long text will make the LLM incautious to the format requirements as the LLM loads query text after sampling instead of reading every word. 

==> tables/table-chat-vs-rag.tex <==
\begin{table*}[!ht]
% \vspace{-6mm}
\caption{
    Complete Performance. 
}
\label{table:performance}
% \setlength{\tabcolsep}{3pt} % Reduce space between columns
\centering
% \footnotesize
% \small
% \resizebox{1.\linewidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c}
\hline
\hline
 & \textbf{\bace} & \textbf{\bbbp} & \textbf{\hiv} 
 & \textbf{\esol} & \textbf{\freesolv} & \textbf{\lipo} \\
\hline
 & \multicolumn{3}{c|}{ROC-AUC $\uparrow$} & \multicolumn{3}{c}{RMSE $\downarrow$} \\
\hline
GCN$^{\CORR}$       & 0.7718 & 0.7045 & 0.7529 & 0.9108 & 2.2102 & 0.7043 \\
GCN$^{\CORR}_{\RAG}$& & & & & & \\
\hline
GIN$^\CORR$         & 0.8214 & 0.6982 & 0.7822 & 0.9137 & 1.9219 & 0.6995 \\
GCN$^{\CORR}_{\RAG}$& 0.6841 & & & & & \\
\hline
\end{tabular}
% }
% \vspace{-5mm}
\end{table*}

==> tables/table-influence-lm.tex <==
\begin{table*}[!ht]
% \vspace{-6mm}
\caption{
    Complete Performance. 
}
\label{table:performance}
% \setlength{\tabcolsep}{3pt} % Reduce space between columns
\centering
% \footnotesize
% \small
% \resizebox{1.\linewidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c}
\hline
\hline
 & \textbf{\bace} & \textbf{\bbbp} & \textbf{\hiv} 
 & \textbf{\esol} & \textbf{\freesolv} & \textbf{\lipo} \\
\hline
 & \multicolumn{3}{c|}{ROC-AUC $\uparrow$} & \multicolumn{3}{c}{RMSE $\downarrow$} \\
\hline
GIN$^\CORR$                 & 0.8214 & 0.6982 & 0.7822 
                            & 0.9137 & 1.9219 & 0.6995 \\
w/o text-embedding-3-small  & 0.8023 & 0.6788 & 0.7699
                            & 0.9276 & 1.9798 & 0.7360 \\
\hline
\end{tabular}
% }
% \vspace{-5mm}
\end{table*}

==> tables/table-k.tex <==
\begin{table*}[!ht]
% \vspace{-6mm}
\caption{
    Complete Performance. 
}
\label{table:performance}
% \setlength{\tabcolsep}{3pt} % Reduce space between columns
\centering
% \footnotesize
% \small
% \resizebox{1.\linewidth}{!}{
\begin{tabular}{l|c|c|c|c}
\hline
\hline
 & \textbf{\bace} & \textbf{\bbbp} 
 & \textbf{\esol} & \textbf{\freesolv} \\
\hline
 & \multicolumn{2}{c|}{ROC-AUC $\uparrow$} & \multicolumn{2}{c}{RMSE $\downarrow$} \\
\hline
GIN$^\CORR$ & 0.8214
            & 0.6982
            & 0.9137
            & 1.9219 \\
k = 30      & 0.7836 
            & 0.6793
            & 0.9518
            & 1.9802 \\
k = 10      & 0.7669
            & 0.5973
            & 0.9821
            & 2.1450\\
\hline
\end{tabular}
% }
% \vspace{-5mm}
\end{table*}
